Bringing Textual Prompt to AI-Generated Image Quality Assessment

AI-Generated Images (AGIs) have inherent multimodal nature. Unlike traditional image quality assessment (IQA) on natural scenarios, AGIs quality assessment (AGIQA) takes the correspondence of image and its textual prompt into consideration. This is coupled in the ground truth score, which confuses the unimodal IQA methods. To solve this problem, we introduce IP-IQA (AGIs Quality Assessment via Image and Prompt), a multimodal framework for AGIQA via corresponding image and prompt incorporation. Specifically, we propose a novel incremental pretraining task named Image2Prompt for better understanding of AGIs and their corresponding textual prompts. An effective and efficient image-prompt fusion module, along with a novel special [QA] token, are also applied. Both are plug-and-play and beneficial for the cooperation of image and its corresponding prompt. Experiments demonstrate that our IP-IQA achieves the state-of-the-art on AGIQA-1k and AGIQA-3k datasets. Code will be available at https://github.com/Coobiw/IP-IQA.

==> intro.tex <==
With the development of deep learning, artificial intelligence (AI) significantly changes the way to generate content. Many impressive AI tools have been developed that can assist in generating content, such as ChatGPT and Stable Diffusion (SD)\cite{rombach2022high}. And the content generated with the assistance of AI technology is referred to Artificial Intelligence Generated Content (AIGC), including images, audios, texts, and videos. Since vision is the the most important way of human perception, vision-related AIGC content, especially AI-Generated Images (AGIs), are becoming prevalent in many fields. Recently, numerous AGI models based on different technical routes have been developed, mainly branched into auto regressive-based models and diffusion-based models. There are several Text-to-Image (T2I) generation models already serving end users, such as Stable Diffusion, Stable Diffusion XL\cite{rombach2022high}, DALLE\cite{ramesh2022hierarchical}, Midjourney, GLIDE\cite{nichol2021glide} and \textit{etc.}, providing different choices for generating images.

As an emerging new image type, AGIs are perceptibly different on several quality-related attributes compared with natural scene images (NSIs). For example, AGIs is statistically more blur because AGIs may occasionally face insufficient iterations during the generation process. AGIs encounter the same low-level distortions that NSIs encounter, such as blur, compression, \textit{etc.}. In addition, AGIs may suffer from some unique impairments such as unnaturalness and unreasonable artifact. When it comes to T2I generation models, the semantic information of the input text prompts relies on the language model, making the correspondence between generated image and text vary. So there are certain distortions about image-text discrepancy, denoting the mismatch between the AGIs and users' expectation. Thus, it is significant to conduct objective image quality assessment (IQA) study for AGIs.

However, existing objective IQA models proposed for NSIs are insufficient for evaluating the quality of AGIs due to the extra dissimilar distortions. The objective models for NSIs consider the low-level distortions of the images, while AGIs suffer from both low-level artifacts and high-level semantic degradations. Every generated image has its corresponding texual prompt, which shows that AGIs have a multimodal nature. Consequently, existing IQA models, taking only the image modality into consideration, are not enough for the quality assessment of AGIs. Considering the correspondence between text prompts and image also makes the AGI quality assessment (AGIQA) model different. As shown in Fig. 1, single-modal models cannot output accurate predictions when the target scores are coupled with the image-prompt correspondence. So, a good AGIQA model needs to take the input of the textual prompt modality into account to give a comprehensive assessment.

To address the problems, a multimodal AGIQA baseline is proposed, which can hanle both image and its corresponding textual prompt, named IP-QA (AG\textbf{I}s \textbf{Q}uality \textbf{A}ssessment via \textbf{I}mage and \textbf{P}rompt). We believe that the incorporation of textual prompt aligns well with the inherently multimodal nature of AGIs.  We hope that IP-IQA will serve as an effective and efficient baseline for AGIQA on multimodal track, for further research purpose. The key contributions of our work can be summarized as following:
\begin{itemize}
    \item IP-IQA is the first work to take both image and textual prompt into consideration for comprehensive assessment, to our best knowledge.
    \item IP-IQA introduces a novel incremental pretraining task, named Image2Prompt, which is significantly beneficial for the model to understand the AGIs and their corresponding prompts.
    \item IP-IQA also proposes an effective and efficient image-prompt fusion module, as well as a special \textit{[QA]} token, which are both plug-and-play. 
    \item IP-IQA achieves the state-of-the-art performance on both AGIQA-1k\cite{zhang2023perceptual} and AGIQA-3k\cite{li2023agiqa}.
    
\end{itemize}

==> problem.tex <==
Given a AGI dataset containing image and corresponding text prompts denoted as $D = \{(\langex_1, t_1\rangle, y_1), ..., (\langlex_n, t_n\rangle, y_n) \}$
